Stablecoins 2.0: Economic Foundations and Risk-based Models

Stablecoins are one of the most widely capitalized type of cryptocurrency. However, their risks vary significantly according to their design and are often poorly understood. We seek to provide a sound foundation for stablecoin theory, with a risk-based functional characterization of the economic structure of stablecoins. First, we match existing economic models to the disparate set of custodial systems. Next, we characterize the unique risks that emerge in non-custodial stablecoins and develop a model framework that unifies existing models from economics and computer science. We further discuss how this modeling framework is applicable to a wide array of cryptoeconomic systems, including cross-chain protocols, collateralized lending, and decentralized exchanges. These unique risks yield unanswered research questions that will form the crux of research in decentralized finance going forward.

==> tables/non-custodial_breakdown.tex <==
\begin{table*}
    \centering
    \begin{tabularx}{\textwidth}{lXXXX}
        \toprule
        \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Primary Value}}\\
        \cmidrule(lr){2-5}\\[-1em]
        {} & \textbf{Exogenous} &  \multicolumn{1}{c}{$\Longleftrightarrow$\hspace*{3em}} & \textbf{Endogenous} & \textbf{Implicit} \\
        \cmidrule{2-5}
        \textbf{Risk-absorber:} agent & \multirow{2}{*}{Dai, Augmint} & \multirow{2}{*}{-} & \multirow{2}{*}{Synthetix, bitUSD} & \multirow{2}{*}{NuBits}\\
        \textbf{Issuance:} agent &   &  &   & \\ \\
        \textbf{Risk-absorber:} equity & \multirow{2}{*}{Duo Network} & \multirow{2}{*}{Steem Dollars, Celo} & \multirow{2}{*}{Terra, USDX, Melmint} & \multirow{2}{*}{Basis (defunct), BitBay} \\
        \textbf{Issuance:} algorithmic &  &  &  & \\ \\
        \textbf{Risk-absorber:} miner & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{Kowala (defunct)}\\
        \textbf{Issuance:} algorithmic &  &  &  & \\
        \bottomrule
    \end{tabularx}
    \caption{Non-custodial stablecoins and applicable models (excluding governance and data feed components).}
    \label{table:non-custodial_breakdown}
\end{table*}



%- Table 2: main-takeaway table of noncustodial stablecoin types (Ari + Dominik?): formatting, is 'equity' right name?, color of issuance dimension

% \begin{table}[h]
%     \centering
%     \begin{tabularx}{\columnwidth}{XXXXX}
%         \toprule
%         % \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Collateral Type}}\\
%         % \cmidrule(lr){2-5}\\[-1em]
%         % {} & Exogenous &  \multicolumn{1}{c}{$\Longleftrightarrow$\hspace*{3em}} & Endogenous & Implicit \\
%         % \midrule
%         % \textbf{Combined agent risk-absorber and issuance} & Dai, Augmint  &  & Synthetix, bitUSD & NuBits \\
%         % \textbf{Equity risk-absorber, algorithmic issuance} & Duo Network & Steem Dollars, Celo & Terra, USDX & Basis (defunct), BitBay, Melmint \\
%         % \textbf{Miner risk-absorber, algorithmic issuance} &  &  &  & Kowala (defunct) \\
%          & \textbf{Risk-absorber/} & Agent/ & Equity/ & Miner/ \\
%       \textbf{Collateral} & \textbf{issuance} & agent & algorithmic & algorithmic \\
%         \midrule
%         Exogenous &  & Dai, & Duo & \\
%           &  & Augmint & Network & \\
%         $\Longleftrightarrow$ &  && Steem Dollars, & \\
%          &   &  & Celo & \\
%         Endogenous &  & Synthetix, & Terra, & \\
%          &   & bitUSD & USDX & \\
%         Implicit &  & NuBits & Basis $^{*}$, & Kowala $^{*}$\\
%         &&& BitBay, & \\
%         &&& Melmint & \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Non-Custodial stablecoins and applicable models. NB $^{*}$ denotes defunct.}
%     \label{table:non-custodial_breakdown_vertical}
% \end{table}

==> tables/non-custodial_deleveraging.tex <==
\begin{table*}
	\begin{tabularx}{\textwidth}{clX}
	    \toprule
		\textbf{Stablecoin}	&   \textbf{Time Period}    &	\textbf{Event} \\
		\midrule
		Maker/Dai	&   Dec. 2018    &	Deleveraging feedback $\implies$ Dai price premium~\cite{dai-premium} \\
		Maker/Dai &   Mar. 2020 &   Deleveraging feedback $\implies$ Dai price premium (`Black Thursday')~\cite{black-thur} \\
		Maker/Dai & Mar. 2020 & Collateral liquidation auctions settle at 0 due to liquidity and congestion~\cite{black-thur} \\
		bitUSD &   Winter 2018-19 &   Broken peg, global settlement due to low collateralization~\cite{bitusd,bitusd-bsip58} \\
% 		bitUSD & Winter 2019-20, ongoing &  \\
% 		bitBTC & Mar. 2019-ongoing & \\
		Steem Dollars & Dec. 2018 & Broken peg, haircut in redeemability due to system debt level~\cite{steemdollar} \\
% 		Steem Dollars & Winter 2019-20 &  \\
		NuBits & Summer 2016 & Crisis of confidence~\cite{nubits-first-blog,nubits-reserve,nubits} \\
		NuBits & Mar. 2018-ongoing & Crisis of confidence, equity position unable to absorb enough supply~\cite{nubits-reserve,nubits} \\
		\bottomrule
	\end{tabularx}
	\caption{Notable non-custodial stablecoin deleveraging events.}
	\label{table:deleveraging_events}
\end{table*}

==> tables/oracle_manipulation.tex <==
\begin{table*}
	\begin{tabularx}{\textwidth}{clX}
	    \toprule
		\textbf{Project}	&   \textbf{Time Period}    &	\textbf{Event} \\ \midrule
		Synthetix	&  Jun. 2019  &	 Error in FX price feed making KRW price skyrocket~\cite{synthetix} \\
		Nuo Network	&   Jun. 2019  & Link token price cannot be correctly read due to single point of failure~\cite{nuo} \\
		Terra	&   Jul. 2019  & The price of Luna/KRW pair on Coinone exchange was manipulated~\cite{terra} \\
		bZx	&   Feb. 2020  & wBTC price on Uniswap was pumped by margin trading on bZx~\cite{bzx1} \\
		bZx	&   Feb. 2020  & sUSD price on KyberSwap and Uniswap was manipulated~\cite{bzx2,bzx-chainlink,bzx-oracle} \\
		\bottomrule
	\end{tabularx}
	\caption{Non-custodial system oracle manipulation events.}
	\label{table:manipulation_events}
\end{table*}
